Beyond Single Items: Exploring User Preferences in Item Sets with the Conversational Playlist Curation Dataset

Users in consumption domains, like music, are often able to more efficiently provide preferences over a set of items (e.g. a playlist or radio) than over single items (e.g. songs). Unfortunately, this is an underexplored area of research, with most existing recommendation systems limited to understanding preferences over single items. Curating an item set exponentiates the search space that recommender systems must consider (all subsets of items!): this motivates conversational approaches-where users explicitly state or refine their preferences and systems elicit preferences in natural language-as an efficient way to understand user needs. We call this task conversational item set curation and present a novel data collection methodology that efficiently collects realistic preferences about item sets in a conversational setting by observing both item-level and set-level feedback. We apply this methodology to music recommendation to build the Conversational Playlist Curation Dataset (CPCD), where we show that it leads raters to express preferences that would not be otherwise expressed. Finally, we propose a wide range of conversational retrieval models as baselines for this task and evaluate them on the dataset.

==> data_eval.table.tex <==
\begin{tabular}{lcc}
\toprule
\textbf{Question}                         & \textbf{MusicRecDialog} & \textbf{CPCD}   \\
\midrule
\textit{How consistent are the preferences?} &                &        \\
\cmidrule{1-1}
Not at all (0)                      & 3.7\%          & 1.0\%  \\
Somewhat (0.5)                      & 16.5\%         & 9.1\%  \\
Very (1)                            & 79.7\%         & 89.8\% \\
Overall                             & 88.0\%         & 94.4\% \\
\midrule
\textit{How relevant is the slate?}        &                &        \\
\cmidrule{1-1}
Not at all (0)                      & 4.8\%          & 1.9\%  \\
Somewhat (0.5)                      & 26.2\%         & 24.1\% \\
Very (1)                            & 68.9\%         & 74.0\% \\
Overall                             & 82.1\%         & 86.0\% \\
\midrule
\textit{How natural is the conversation?}    &                &        \\
\cmidrule{1-1}
Not at all (0)                      & 3.0\%          & 0.3\%  \\
Somewhat (0.5)                      & 46.2\%         & 35.3\% \\
Very (1)                            & 50.8\%         & 64.4\% \\
Overall                             & 73.9\%         & 82.0\% \\
\toprule
\end{tabular}

==> figures/music-survey.table.tex <==
\begin{tabular}{l rrrr rrrr} \toprule
         & \multicolumn{4}{c}{Users (110)} & \multicolumn{4}{c}{Wizards (10)} \\
\midrule
\multicolumn{9}{l}{\textit{In which of the following contexts do you typically listen to music?}} \\
In the car & \multicolumn{4}{r}{88.9\%} & \multicolumn{4}{r}{100\%} \\
Relaxing at home & \multicolumn{4}{r}{94.4\%} & \multicolumn{4}{r}{90\%} \\
Commuting to work / school & \multicolumn{4}{r}{65.2\%} & \multicolumn{4}{r}{100\%} \\
Cooking and cleaning (or other chores) & \multicolumn{4}{r}{85.4\%} & \multicolumn{4}{r}{100\%} \\
Working / studying & \multicolumn{4}{r}{74.1\%} & \multicolumn{4}{r}{60\%} \\
Exercising / at the gym & \multicolumn{4}{r}{80\%} & \multicolumn{4}{r}{80\%} \\
Going to sleep & \multicolumn{4}{r}{55.1\%} & \multicolumn{4}{r}{30\%} \\
\midrule
\multicolumn{9}{l}{\textit{How familiar are you with the following genres of music?}} \\
    & Not at all & \cdot & \cdot & Very & Not at all & \cdot & \cdot & Very \\
    \cmidrule{2-5,6-9}
R\&B / Hip-Hop / Rap
    & 2\% & 8\% & 15\% & 75\%
    & 0\% & 20\% & 35\% & 45\% \\
Rock
    & 2\% & 12\% & 23\% & 62\%
    & 15\% & 10\% & 30\% & 45\% \\
Pop	&
    & 1\% & 7\% & 22\% & 70\%
    & 0\% & 10\% & 55\% & 35\% \\
Country &
    & 8\% & 21\% & 25\% & 45\%
    & 25\% & 25\% & 35\% & 15\% \\
Latin	 &
    & 30\% & 28\% & 18\% & 23\%
    & 45\% & 40\% & 10\% & 5\% \\
Electronic / Dance  &
    & 13\% & 23\% & 28\% & 37\%
    & 15\% & 50\% & 25\% & 10\% \\
Religious (Christian, Gospel, etc.)	&
    & 19\% & 16\% & 20\% & 45\%
    & 55\% & 25\% & 10\% & 10\% \\
Holiday / Seasonal	 &
    & 4\% & 15\% & 32\% & 49\%
    & 10\% & 35\% & 35\% & 20\% \\
Children	 &
    & 14\% & 27\% & 27\% & 33\%
    & 60\% & 15\% & 15\% & 10\% \\
Jazz	 &
    & 14\% & 22\% & 23\% & 40\%
    & 25\% & 45\% & 25\% & 5\% \\
Classical &
    & 11\% & 22\% & 22\% & 44\%
    & 40\% & 35\% & 15\% & 10\% \\
\bottomrule
\end{tabular}


% Users 
% How frequently do you listen to music?
% A few times a month or less
% 1 & 2 & 3 & 4 & 5
% Multiple times a day
% 0.2\% & 0.5\% & 2.4\% & 9\% & 87.8\%

% How passionate are you about music?
% Not at all
% Extremely passionate
% 1 & 2 & 3 & 4 & 5
% 0 & 0.2 & 3.9 & 16.5 & 79.3

% In which of the following contexts do you typically listen to music?
% In the car 88.9%
% Relaxing at home 94.4%
% Commuting to work / school 65.2%
% Cooking and cleaning (or other chores) 85.4%
% Working / studying 74.1%
% Exercising / at the gym 80%
% Going to sleep 55.1%

% How familiar are you with the following genres of music?
% R\&B / Hip-Hop / Rap & 18 & 67 & 123 & 614 \\
% Rock	& 17 & 102 & 193  & 510 \\
% Pop	& 6 & 55 & 183 & 578  \\
% Country & 67 & 178 & 208 & 375 \\
% Latin	 & 249 & 232 & 152 & 189 \\
% Electronic / Dance  & 104 & 189 & 228 & 301 \\
% Religious (Christian, Gospel, etc.)	& 160 & 130 & 161 & 371 \\
% Holiday / Seasonal	 & 33 & 122 & 263 & 404 \\
% Children	 & 114 & 218 &  222 & 268 \\
% Jazz	 & 114 & 184 & 192 & 332 \\
% Classical & 94 & 184 & 182 & 362 \\



% Wizard
% How frequently do you listen to music?
% A few times a month or less
% 1 & 2 & 3 & 4 & 5
% Multiple times a day
% 0\% & 0\% & 0\% & 25\% & 75\%

% How passionate are you about music?
% Not at all
% Extremely passionate
% 1 & 2 & 3 & 4 & 5
% 0 & 0 & 10 & 40 & 50

% In which of the following contexts do you typically listen to music?
% In the car 100%
% Relaxing at home 90%
% Commuting to work / school 100%
% Cooking and cleaning (or other chores) 100%
% Working / studying 60%
% Exercising / at the gym 80%
% Going to sleep 30%

% How familiar are you with the following genres of music?
% R & B / Hip-Hop / Rap	 & 0 & 4 & 7 & 9
% Rock	& 3 & 2 & 6 & 9
% Pop	& 0 & 2 & 11 & 7
% Country & 5 & 5 & 7 & 3
% Latin	 & 9 & 8 & 2 & 1
% Electronic / Dance  & 3 & 10 & 5 & 2
% Religious (Christian, Gospel, etc.)	& 11 & 5 & 2 & 2
% Holiday / Seasonal	 & 2 & 7 & 7 & 4
% Children	 & 12 & 3 & 3 & 2
% Jazz	 & 5 & 9 & 5 & 1
% Classical & 8 & 7 & 3 & 2

